RoboTurk: A Crowdsourcing Platform for Robotic Skill Learning through Imitation

Imitation Learning has empowered recent advances in learning robotic manipulation tasks by addressing shortcomings of Reinforcement Learning such as exploration and reward specification. However, research in this area has been limited to modest-sized datasets due to the difficulty of collecting large quantities of task demonstrations through existing mechanisms. This work introduces RoboTurk to address this challenge. RoboTurk is a crowdsourcing platform for high quality 6-DoF trajectory based teleoperation through the use of widely available mobile devices (e.g. iPhone). We evaluate RoboTurk on three manipulation tasks of varying timescales (15-120s) and observe that our user interface is statistically similar to special purpose hardware such as virtual reality controllers in terms of task completion times. Furthermore, we observe that poor network conditions, such as low bandwidth and high delay links, do not substantially affect the remote users' ability to perform task demonstrations successfully on RoboTurk. Lastly, we demonstrate the efficacy of RoboTurk through the collection of a pilot dataset; using RoboTurk, we collected 137.5 hours of manipulation data from remote workers, amounting to over 2200 successful task demonstrations in 22 hours of total system usage. We show that the data obtained through RoboTurk enables policy learning on multi-step manipulation tasks with sparse rewards and that using larger quantities of demonstrations during policy learning provides benefits in terms of both learning consistency and final performance. For additional results, videos, and to download our pilot dataset, visit $\href{http://roboturk.stanford.edu/}{\texttt{roboturk.stanford.edu}}$

==> 0-preamble.tex <==
% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.

% ---------------------------------
%ISRR dependencies 
% ---------------------------------
\usepackage{helvet}
\usepackage{courier}
\usepackage{graphicx}
\usepackage{makeidx}
\usepackage{multicol}
\usepackage[bottom]{footmisc}%place footnotes at the bottom


% ---------------------------------
%floats and figures
% ---------------------------------
%\usepackage{graphics}
%\usepackage[pdftex]{graphicx}
%\usepackage{wrapfig}
%\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200

% \usepackage[font={small}]{caption}
\usepackage{subcaption}
\captionsetup{compatibility=false}
%\usepackage[center]{subfigure} %DONT USE BOTH SUBCAPTION AND SUBFIGURE
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

% ---------------------------------
%Math Stuff
% ---------------------------------
\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\let\proof\relax
\let\endproof\relax 
\usepackage{amsthm}
\usepackage{ wasysym } %special symbols
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{mathptmx} % selects Times Roman as basic font
\usepackage{gensymb} 
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{mdwmath}
% \usepackage{mdwtab}
% \usepackage{eqparbox} %equations

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
%\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

\usepackage{algorithm} %float wrapper for algorithms.%dont use with algorithm2e

\usepackage{algorithmic} %least preferred
\floatname{algorithm}{Algorithm}
\renewcommand{\algorithmiccomment}[1]{// #1}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

%should only use one of algorithmic or algorithmicx or algorithm2e
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
% \usepackage{algorithmicx, algpseudocode} %algpseudocode:layout for algorithmicx

% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{booktabs}       % professional-quality tables
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}

% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc} 
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
% \usepackage{siunitx}
\usepackage{bm}
\usepackage{times} % assumes new font selection scheme installed
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
% \usepackage[yyyymmdd,hhmmss]{datetime}
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{enumitem}
% \setlist[enumerate]{itemsep=0mm}
% \usepackage{enumerate}
% \let\labelindent\relax

% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

%\usepackage[protrusion=true,expansion=true]{microtype}
% \setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
\usepackage{url}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
\usepackage[usenames,dvipsnames,table]{xcolor}

% hyperref already loaded in corl file -- dont load again
% \usepackage[pdfborder={0 0 0.5},bookmarks=false]{hyperref}

\hypersetup{
    colorlinks=true,
    linkcolor=black,
    citecolor=mydarkblue,
    filecolor=cyan,
    urlcolor=black
}

%=======U S E R  D E F I N E D  M A C R O S=======
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}

% \newcommand{\todo}[1]{}
\newcommand{\todo}[1]{\textcolor{red}{[#1?]}}
\newcommand{\todoJH}[1]{\textcolor{blue}{[JH:#1]}}

\newcommand{\tocite}[1]{\textcolor{red}{[cite:#1?]}}
\newcommand{\ignore}[1]{}
% \newcommand{\del}[1]{}

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it

\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter~\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}


% \newtheorem{theorem}{Theorem}
% \newtheorem{example}{Example}
% \newtheorem{definition}{Definition}
% \newtheorem{problem}{Problem}
% \newtheorem{property}{Property}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}

%version in control in draft mode
% Simple and headings are two pagestyles in the ucbthesis class. May need edits to whatever different pagestyle is being used. 
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}


% ---------------------------------
%   SPACE TWEAKS 
% ---------------------------------
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{0.5mm} 
\setlength{\textfloatsep}{1mm}
\setlength{\dbltextfloatsep}{1mm}
% \renewcommand{\baselinestretch}{.9945}

\usepackage{titlesec}
\titlespacing*{\section}
{0pt}{.4\baselineskip}{0.5\baselineskip}
\titlespacing*{\subsection}
  {0pt}{0.25\baselineskip}{0.2\baselineskip}

==> 1-intro-v2.tex <==

%===========================================================================
\vspace{-5pt}
\section{Introduction}
\vspace{-5pt}

Research in computer vision and natural language processing has benefited immensely from very large scale supervised datasets~\cite{deng2009imagenet,lin2014microsoft,rajpurkar2018squad2}. Structured labeling of data in problems such as image classification, and machine translation have not only provided a fertile ground for development of a broad set of algorithms, but also boosted progress via benchmarking. This paper is an attempt to create a framework for scalable crowd-sourced method to detailed supervision for manipulation skills that in turn can potentially enable efficient skill learning. We use consumer grade hardware coupled with cloud run simulation framework to ensure homogeneous quality of service for citizen scientists. 

Along similar lines, supervised data is very helpful in policy learning for robotics. 
% Imitation learning is more efficient than RL 
Prior works in robot learning have leveraged Reinforcement Learning (RL) and Imitation Learning (IL) successfully for short-horizon skill learning such as learning to push and grasp objects~\cite{yu2016more,levine2016learning}. However, RL methods face the burden of exploring a large state space efficiently, specifying of reward, and need large amounts of interaction with the environment. In contrast, IL attempts to use demonstrations provided by an expert to circumvent these issues and guide an agent to learn to accomplish skills efficiently with smaller amounts of environment interaction. 
Imitation based mechanisms in robot policy learning have shown to be more effective than exploratory model-free reinforcement learning (RL)~\cite{gupta2016learning,boularias2011relative,krishnan2016swirl,ho2016generative}. 
Prior work has shown that the use of expert data can improve the sample efficiency of policy learning not only in conventional RL algorithms like apprenticeship learning~\cite{abbeel2010autonomous} but also in recent deep RL algorithms such as DDPGfD~\cite{vevcerik2017leveraging}.

% LfD for imitation is popular and there are many mechanisms of getting data. 
Imitation Learning is commonly posed either in the inverse reinforcement learning~\cite{abbeel2011inverse,ng2000algorithms} or behaviour cloning framework~\cite{argall2009survey,pomerleau1989alvinn}. In both cases, demonstrations are frequently provided through kinesthetically guiding a robot through a desired trajectory. Albeit intuitive, this mechanism of data collection is limited to a small number of demonstrations, often of the order of tens, partially due to the tedious mechanism of supervision. 
Moreover, the actual number of trajectories required for LfD can often be much larger than a few dozen~\cite{osentoski2010crowdsourcing}. 
The robotics community has explored large-scale data-driven approaches for grasping using cloud based systems for both computations~\cite{mahler2017dex,kasper2012kit,goldfeder2009columbia} and physical self-supervision for learning to grasp~\cite{levine2016learning,pinto2016supersizing}. While reasonably large in scale, the data acquired has little signal to noise ratio due to random exploration. Hence a better initialization of policies from imitation can yield improved performance of physical interaction. 

In domains outside of robotics, large-scale supervision for datasets is often collected with the assistance of crowdsourced workers~\cite{deng2009imagenet,rajpurkar2018squad2}. This enables a scalable mechanism for diverse human supervision on an extensive set of problem instances. However, collecting large amounts of data has been a challenge for continuous manipulation tasks. 
The need for increasing amounts of supervised data from crowdsourced workers led to the use of teleoperation-based techniques~\cite{Goldberg94beyondthe,sung2018robobarista,hokayem2006bilateral}. Teleoperated supervision can be provided through (a) \textit{game interfaces} such as a video-game controller~\cite{laskey2017comparing}, a keyboard-and-mouse~\cite{kent2017comparison}, a point-and-click~\cite{leeper2012strategies}, a 3D-mouse~\cite{Dragan-2012-7572}, and (b) \textit{free-space positioning interfaces} such as Phantom Omni~\cite{akgun2012novel}, da Vinci surgical robot~\cite{liang2017using} and virtual reality (VR)~\cite{whitney2017comparing,zhang2017deep,lipton2018baxter}. These interfaces span a spectrum of capabilities in terms of allowing the user to control a subset of robot's available degrees of freedoms. Additionally, general purpose hardware for game interfaces frequently introduces artifacts in trajectories that reduce utility of this data for imitation~\cite{akgun2012keyframe}. For instance, due to concurrent control of only a subspace of actions, the trajectories can be longer, exhibit axis-aligned movement, and lack the natural variations in motion.

% natural 6-DoF variations between trajectories across examples and problem instances are not captured in game interfaces with concurrent control of only a subspace of available actions \todo{clean this up, talk about axis-aligned movements, and ease of use/operation}. 

% existing mechanism limit the data collection and do not provide true crowdsourcing. 
% Dextrous manipulation in the dull, dirty and dangerous environs have the potential to improve quality of life for human operators. Since the current techniques fall short of complete automation in these settings, intervention of human expert through teleoperated supervision is often an effective alternative that allows the operators to utilize the semantic and contextual expertise to the task. 

% dirty dull dangerous. 
% Teleoperation allows a human to remotely operate a robot to perform complex and potentially dangerous tasks such as defusing a bomb, repairing a nuclear reaction, or maintaining the exterior of a space station

Virtual Reality (VR) controllers have attracted efforts for robot control~\cite{lipton2018baxter,whitney2017comparing}.
Free-space positioning interfaces such as VR enable the user to directly move the robot’s end effector by moving a hand controller in 3D space, enabling fine-grained dexterous control. 
Interestingly, Zhang et al.~\cite{zhang2017deep} showed that simpler algorithms such as variants of behavior cloning can be made to learn short-horizon manipulation tasks with data from VR demonstrations.
However this required collocation with the robot using specialized hardware and a single user was limited to hundreds of demonstrations. 
To empower learning algorithms for robots to accomplish longer-horizon manipulation tasks and generalize across different tasks, it is necessary to gather larger variations of supervised data. 

While these methods have shown the utility of data, they do not provide a seamlessly scalable data collection mechanism. The data is collected locally, and also requires a powerful local client computer to render the high-definition sensor stream to a VR headset~\cite{whitney2017comparing, zhang2017deep}.
Despite the popularity of VR headsets and controllers, they are yet to be a commodity hardware. It is, in fact, a special purpose gaming accessory that caters to a niche audience of gaming users, who are often not representative of workers on crowdsourcing platforms.
For example, only 400K units of HTC Vive sold in 2016 compared to 211 million new iPhone units sold in 2016 alone~\cite{superdata2017vr,apple2017report}. This has limited the use of VR for teleoperation to controlled workstations as opposed to being ubiquitous and suitable for crowdsourcing~\cite{zhang2017deep,whitney2017comparing}. 
Consequently, the use of VR hardware and requirement of client-side compute resources has limited the deployment of these interfaces on crowd-sourcing platforms such as Amazon Mechanical Turk. 

% However, these methods have only been able to leverage on the order of 100s of demonstrations due to limits on data collection capacity and requirement of specialized hardware. 

% \todo{super linear growth, completion times for Pieter's tasks, need longer horizon task demonstrations, generalization, etc}
% However, methods such as in \tocite{} require hundreds of demonstrations for relatively short horizon manipulation tasks. 


% VR is not happening fast enough. the intended user doesnt actually have a game assesory. while it is more accurate we show that with a bit of clever design we can get similar accuracy but much larger userbase.


\begin{figure*}[!t]
\centering
\begin{minipage}[t]{0.495\linewidth}
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{figures/system_image.png}
    \vspace{-5pt}
\end{minipage}%
\begin{minipage}[t]{0.495\linewidth}
    \centering
    \vspace{-5pt}
    \includegraphics[width=\linewidth]{figures/sys_diagram.png}
    \vspace{-5pt}
\end{minipage}%
    \vspace{-10pt}
\caption{\textbf{System Overview}: \textbf{Left}: the user interface elements of \sysAbbr{} that were used throughout our evaluation. \textbf{Right}: system diagram of \sysAbbr{}. The process for collecting a demonstration with \sysAbbr{} is as follows: (1) Users connect to a web front-end and authenticate with the system. (2) A coordination server helps to establish a direct communications channel between the user's web browser \& iPhone and an available robot simulator instance. (3) Coordination server severs connection with user; user communicates with the robot simulator instance directly for the duration of the session. (4) After each successfully demonstration is completed, the robot simulator instance pushes the associated data to a storage system.}
  \label{fig:sys_diagram}
\vspace{-15pt}
\end{figure*}

% \todo{highlight the component of on-demand, we need a data collection SYSTEM}

% It is highly unlikely that a single dataset will be able to solve these challenges. There is significant variation across robots, task definitions, objects, and surroundings. This motivates the need for a data collection \textit{system} that is \textit{dynamic} and able to produce large quantities of data to help robots generalize to diverse environment conditions. To address this need, we propose a novel crowdsourcing system for collecting demonstrations to complete challenging domain-specific robotics tasks.

This paper proposes a systematic framework to address the challenge of cloud-enabled crowd-sourcing from large-scale and on-demand workers to provide trajectory level training input in robot manipulation tasks. We term the proposed framework as \sysFull (\sysAbbr). \sysAbbr is a unified on-demand task-based data collection framework that uses a phone based controller coupled with a web interface for video feedback. 
% Leveraging widely available consumer hardware (>iphone 6s) broadens potential worker base for \sysAbbr, enabling crowdsourcing on commercial platforms. 
We also develop a cloud run simulation framework to ensure homogeneous quality of service regardless of client's compute resources. \sysAbbr relaxes the requirement to have a heavy-duty local computer at the client node. 
The two components combined result in a platform that is intuitive to use, and has a low barrier to entry -- the core requirements of a crowdsourced task.
\sysAbbr enables: (a) real-time control of simulated systems, (b) accessibility to large population of users, and (c) scalable system to accommodate many concurrent users. As a framework, \sysAbbr is one of the first systems to facilitate crowdsourcing of trajectory-level supervision on commercial platforms. 
% The use of consumer hardware already available to a typical user reduces the entry barrier, enabling a much broader scale, true to sense crowdsourcing for robotics as has benefited other areas of machine learning. 

\noindent \textbf{Contributions.} The main contributions of this paper are:
\vspace{-5pt}
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    % partopsep=1ex,
    % parsep=1ex,
    leftmargin=*,
    itemindent=3ex]
\item We develop \sysAbbr{} as a crowdsourcing platform to provide task demonstrations in simulated domains through high-quality 6-DoF supervisory input with a free-space positioning interface using an iPhone as a controller.
\item We conduct a user study comparing the performance of three other interfaces, including a VR interface, on simulated bin sorting and peg-in-hole tasks. Our system is statistically similar to VR in performance and better than 3D-mouse and keyboard interfaces. We also evaluate the performance of \sysAbbr under poor network conditions using a network simulator.
\item We also present an initial dataset consisting of 1280 task demonstrations, amounting to 104 hours of data collected in two days with contracted workers. 
\item We present some initial findings that show that the large amount of data collected is useful in improving convergence rates of policy learning with reinforcement, and that the data obtained through \sysAbbr{} can enhance the performance of policy learning with RL methods.
\end{enumerate}

% We evaluated our interface on a cup-stacking manipulation task with 18 users, comparing the relative effectiveness of a keyboard and mouse interface, virtual reality camera control, and positional hand tracking. Our system reduces task completion time by 101 seconds (a reduction of 66\%), while improving subjective assessments of system usability and workload. Additionally, we have shown the effectiveness of our system over long distances, successfully completing a cup stacking task from over 40 miles away. Our paper contributes a quantitative assessment of robot grasping teleoperation across desktop and virtual reality interfaces. 



==> 1-intro.tex <==

%===========================================================================
\section{Introduction}

Researchers in applications of machine learning such as computer vision and natural language have benefited immensely from very large scale supervised datasets~\cite{deng2009imagenet,lin2014microsoft,rajpurkar2018squad2}. Structured labeling of data in problems such as visual recognition and machine translation have not only provided a fertile ground for development of a broad set of algorithms but also boosted progress through benchmarking. 

Along similar lines, supervised data has been very helpful in policy learning for robotics. 
% Imitation learning is more efficient than RL 
Prior works in robot learning have leveraged Reinforcement Learning (RL) and Imitation Learning (IL) successfully for short-horizon skill learning such as learning to push and grasp objects~\cite{yu2016more,levine2016learning}. However, RL methods face the burden of exploring a large state space efficiently and suffer from a need for large amounts of interaction with the environment. In contrast, IL attempts to use demonstrations provided by an expert to circumvent these issues and guide an agent to learn to accomplish skills efficiently with smaller amounts of environment interaction. 
Imitation based mechanisms in robot policy learning have shown to be more effective than exploratory model-free reinforcement learning (RL). 
Research has shown that the use of expert data can improve the sample efficiency of policy learning not only in conventional RL algorithms like apprenticeship learning~\cite{abbeel2010autonomous} but also in recent deep RL algorithms such as DDPGfD~\cite{vevcerik2017leveraging}.

% LfD for imitation is popular and there are many mechanisms of getting data. 
Imitation Learning is commonly posed either in the inverse reinforcement learning or behaviour cloning framework~\cite{argall2009survey}. In both cases, demonstrations are frequently provided through kinesthetically guiding a robot through a desired trajectory. Albeit intuitive, this mechanism of data collection is limited to a small number of demonstrations, often of the order of tens, partly due to the tedious mechanism of supervision. 
Moreover, the actual number of trajectories required for LfD can often be much larger than a few dozen~\cite{osentoski2010crowdsourcing}. In domains outside of robotics, large-scale supervision for datasets is often collected with the assistance of crowdsourced workers~\cite{deng2009imagenet,rajpurkar2018squad2}. This enables a scalable mechanism for diverse human supervision on an extensive set of problem instances.  

The need for increasing amounts of supervised data from crowdsourced workers led to the use of teleoperation based techniques~\cite{Goldberg94beyondthe,sung2018robobarista,hokayem2006bilateral}. Teleoperated supervision can be provided through (a) \textit{game interfaces} such as a video-game controller~\cite{laskey2017comparing}, a keyboard-and-mouse~\cite{kent2017comparison}, a point-and-click~\cite{leeper2012strategies}, a 3D-mouse~\cite{Dragan-2012-7572}, and (b) \textit{free-space positioning interfaces} such as phantom omni~\cite{akgun2012novel}, da Vinci surgical robot~\cite{liang2017using} and virtual reality (VR)~\cite{zhang2017deep}. These interfaces span a spectrum of capabilities in terms of allowing the user to control a subset of robot's available degrees of freedoms. Additionally, game interfaces frequently introduce artifacts in trajectories that reduce utility of this data for imitation~\cite{akgun2012keyframe}. For instance, due to concurrent control of only a subspace of actions, the trajectories can be longer, exhibit axis-aligned movement, and lack the natural variations in motion. 

% natural 6-DoF variations between trajectories across examples and problem instances are not captured in game interfaces with concurrent control of only a subspace of available actions \todo{clean this up, talk about axis-aligned movements, and ease of use/operation}. 

% existing mechanism limit the data collection and do not provide true crowdsourcing. 
% Dextrous manipulation in the dull, dirty and dangerous environs have the potential to improve quality of life for human operators. Since the current techniques fall short of complete automation in these settings, intervention of human expert through teleoperated supervision is often an effective alternative that allows the operators to utilize the semantic and contextual expertise to the task. 

% dirty dull dangerous. 
% Teleoperation allows a human to remotely operate a robot to perform complex and potentially dangerous tasks such as defusing a bomb, repairing a nuclear reaction, or maintaining the exterior of a space station

Interestingly, Zhang et al.~\cite{zhang2017deep} showed that simpler algorithms such as variants of behavior cloning can be made to learn short-horizon manipulation tasks with data from VR based interfaces. 
However this required collocation with the robot using specialized hardware and a single user was limited to about 100 demonstrations. 
% However, these methods have only been able to leverage on the order of 100s of demonstrations due to limits on data collection capacity and requirement of specialized hardware. 
To empower learning algorithms for robots to accomplish longer-horizon manipulation tasks and generlize to different task instances, it is necessary to gather larger variations of supervised data. 
% \todo{super linear growth, completion times for Pieter's tasks, need longer horizon task demonstrations, generalization, etc}
% However, methods such as in \tocite{} require hundreds of demonstrations for relatively short horizon manipulation tasks. 


% VR is not happening fast enough. the intended user doesnt actually have a game assesory. while it is more accurate we show that with a bit of clever design we can get similar accuracy but much larger userbase.
Virtual reality (VR) controllers have attracted efforts for robot control~\cite{lipton2018baxter,whitney2017comparing}.
Free-space positioning interfaces such as VR enable the user to directly move the robot’s end effector by moving a hand controller in 3D space, enabling fine-grained dexterous control. 
However, despite the popularity of VR headsets and controllers, they are yet to be a commodity hardware. It is, in fact, a special purpose gaming accessory that caters to a niche audience of gaming users, who are often not representative of workers on crowdsourcing platforms.
For example, only 400K units of HTC Vive sold in 2016 compared to 211 million new iphone units sold in 2016 alone~\cite{superdata2017vr,apple2017report}. This has limited the use of VR for teleoperation to controlled workstations as opposed to being ubiquitious and suitable for crowdsourcing~\cite{zhang2017deep,whitney2017comparing}. 


% \todo{highlight the component of on-demand, we need a data collection SYSTEM}

% It is highly unlikely that a single dataset will be able to solve these challenges. There is significant variation across robots, task definitions, objects, and surroundings. This motivates the need for a data collection \textit{system} that is \textit{dynamic} and able to produce large quantities of data to help robots generalize to diverse environment conditions. To address this need, we propose a novel crowdsourcing system for collecting demonstrations to complete challenging domain-specific robotics tasks.

\begin{figure*}[!t]
\centering
\begin{minipage}[t]{0.495\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/system_image.png}
\end{minipage}%
\begin{minipage}[t]{0.495\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/sys_diagram.png}
\end{minipage}%
\caption{LEFT: the user interface elements of \sysAbbr{} that were used throughout our evaluation. RIGHT: system diagram of \sysAbbr{}. The process for collecting a demonstration with \sysAbbr{} is as follows: (1) Users connect to a web frontend and authenticate with the system. (2) A coordination server helps to establish a direct communications channel between the user's web browser \& iPhone and an available robot simulator instance. (3) Coordination server severs connection with user; user communicates with the robot simulator instance directly for the duration of the session. (4) After each successfully demonstration is completed, the robot simulator instance pushes the associated data to a storage system.}
  \label{fig:sys_diagram}
\end{figure*}

This paper proposes a systematic framework to address the challenge of cloud-enabled crowd-sourcing from large-scale and on-demand workers to provide trajectory level training input in robot manipulation tasks. We term the proposed framework as \sysFull (\sysAbbr). \sysAbbr is a unified on-demand task-based data collection framework that uses a phone based controller coupled with a web interface for video feedback. 
% Leveraging widely available consumer hardware (>iphone 6s) broadens potential worker base for \sysAbbr, enabling crowdsourcing on commercial platforms. 
\sysAbbr enables: (a) real-time control of simulated systems, (b) accessibility to large population of users, and (c) scalable system to accommodate many concurrent users. As a framework, \sysAbbr is one of the first systems to facilitate crowdsourcing of trajectory level detailed supervision on commercial platforms. 
% The use of consumer hardware already available to a typical user reduces the entry barrier, enabling a much broader scale, true to sense crowdsourcing for robotics as has benefited other areas of machine learning. 

\noindent \textbf{Contributions.} The main contributions of this paper are:
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    % partopsep=1ex,
    % parsep=1ex,
    leftmargin=*,
    itemindent=3ex]
\item We develop the \sysFull framework as a crowdsourcing platform to provide task demonstrations in simulated domains through high quality 6-DoF supervisory input with a free-space positioning interface using an iPhone as a controller. 
\item We present results of a user study evaluation comparing the performance of three other interfaces, including a VR interface, on simulated sequential pick-and-place and peg-in-hole tasks. Our system is statistically similar to VR in performance and better than 3D-mouse and keyboard interfaces. We also evaluate the performance of \sysAbbr under poor network conditions using a network simulator.
\item We also present an initial dataset of over 100 hours of data collected in two days on our platform from contracted workers employed in China. 
\item We present some initial findings that show that the large amount of data collected is useful in improving convergence rates of policy learning with reinforcement, and that policies trained using this data outperform reinforcement learning approaches.
\end{enumerate}

% We evaluated our interface on a cup-stacking manipulation task with 18 users, comparing the relative effectiveness of a keyboard and mouse interface, virtual reality camera control, and positional hand tracking. Our system reduces task completion time by 101 seconds (a reduction of 66\%), while improving subjective assessments of system usability and workload. Additionally, we have shown the effectiveness of our system over long distances, successfully completing a cup stacking task from over 40 miles away. Our paper contributes a quantitative assessment of robot grasping teleoperation across desktop and virtual reality interfaces. 



==> 2-rw.tex <==
% % Stacking with visual State
% \begin{figure*}[!t]
% \centering
% \begin{minipage}[t]{.6\linewidth}
%     \centering
%     \vspace{-5pt}
%     \includegraphics[width=\linewidth]{figures/sys_diagram.png}
%     \includegraphics[width=0.9\linewidth]{figures/system_image.png}
%     \vspace{-5pt}
% \end{minipage}%
% \begin{minipage}[t]{.395\linewidth}
%     \centering
%     % \vspace{-5pt}
%     \caption{ {\scriptsize A system diagram that highlights the modular design of \sysAbbr and the process that enables a new user to use our remote teleoperation system. (1) Users connect to a frontend server to authenticate themselves to the system. (2) Users then connect to a coordination server that helps establish a direct connection between them and the teleoperation server, which hosts a robot in a simulated physics engine. The worker's web browser and iPhone each make separate direct connections to the teleoperation server. (3) Users terminate their connection to the coordination server and communicate with the teleoperation server directly for the duration of the session. (4) After the user successfully completes a demonstration, the teleoperation server pushes the demonstration data to a backend storage system.}}
%     \label{fig:sys_diagram}
%     \vspace{-5pt}
% \end{minipage}%
% \vspace{-20pt}
% \end{figure*}

\section{Related Work}

% RoboBrain~\cite{saxena2014robobrain}
% -Large scale knowledge engine for robotics

% RoboEarth (WWW for robotics)~\cite{waibel2011roboearth}
% networked robots with a database of shared knowledge
%  It envisioned “a World Wide Web for robots: a giant network and database repository where robots can share information and learn from each other about their behavior and environment”

% Rapyuta: A Cloud Robotics Platform~\cite{mohanarajah2015rapyuta}

% DAvinCi: A Cloud Computing Framework for Service Robots~\cite{arumugam2010davinci}

% Off the Shelf Cloud Robotics for the Smart Home: Empowering a Wireless Robot through
% Cloud Computing~\cite{ramirez2017off}
% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5375811/

% DexNet 1.0 ~\cite{mahler2016dex}
% -Uses google cloud to run several simulator instances to train grasping models.


\noindent \textbf{Learning from Demonstration and Imitation Learning}
Imitation learning is a popular approach for efficient policy learning. 
Specification of reward/cost functions can be non-intuitive to design for a number of robotic tasks~\cite{ng2000algorithms}.
Imitation learning can be performed mainly through inverse reinforcement learning (IRL)\cite{abbeel2011inverse} or behavioral cloning (BC)\cite{pomerleau1989alvinn}.
Approaches based on IRL learn a reward function that is consistent with the assumption that a near-optimal expert provided the demonstrations~\cite{abbeel2010autonomous,calinon2009statistical,gupta2016learning,boularias2011relative,krishnan2016swirl,ho2016generative}.
In contrast, BC uses supervised learning to directly learn a mapping from observations to actions~\cite{schulman2016learning, phillips2016learning, ross2013learning, james2017transferring, xu2018neural}
Recent works show that expert trajectories can also be used as training data for off-policy algorithms such as DDPG~\cite{vevcerik2017leveraging}.
% or in an adversarial reward learning setting \cite{ho2016generative}. 
However, these algorithms either require a large amount of data (BC) or a high number of environment interactions (IRL). 

% Rajeswaran et al. [37], Nair et al. [30] both use human demonstrations to aid exploration.
% Most of these methods require observation and/or action spaces to be aligned between the robot and demonstrations.

\noindent \textbf{Large-Scale Data collection in Robotics.}
Robotics research has explored data-driven methods for learning in a number of problems. 
Specifically, grasping has benefit greatly from the use of large-scale data-driven approaches. 
Efforts such as the Columbia grasp database~\cite{goldfeder2009columbia} and the KIT object models database~\cite{kasper2012kit} focused on collecting shape models and evaluating them for manipulation. On the other hand, large scale physical trials of object grasping resulted in a jump in accuracy~\cite{levine2016learning,pinto2016supersizing}. DexNet 2.0~\cite{mahler2017dex} uses a combination of simulation and real trials to improve grasping success even further. Similar attempts were also made for skills such as planar pushing~\cite{yu2016more}. 
The methods above used hundreds of hours of robot interaction, with a majority of those trials not being effective.
Hence a better initialization of policies from imitation can yield improved performance of physical interaction. 

\noindent \textbf{Crowdsourced Teleoperation for Robot Learning}
Collecting large amounts of data has been a challenge for continuous manipulation tasks. Crowdsourcing supervision has resulted in some remarkable scaling of datasets in computer vision and natural language\cite{deng2009imagenet,rajpurkar2018squad2}.  
% Also, kinesthetic teaching can result in visual artifacts and is infeasible at internet scale~\cite{akgun2012keyframe}.
% Laskey et al~\cite{laskey2017comparing} showed that learning from large datasets may be result in improved convergence compared to interactive online corrections as proposed in~\cite{ross2013learning}. 
In Robotics, crowdsourcing over the internet was first introduced to robotics in the Telegarden Project~\cite{Goldberg94beyondthe}.
Since then a number of studies have leveraged the crowd to \textit{ask for help}~\cite{Sorokin-2010-10559,sung2018robobarista,hokayem2006bilateral}. Prior works have also built frameworks for web-based low-latency robot control~\cite{toris2014robot}.  Kehoe et al.\cite{kehoe2014tase} provides an excellent treatise that touches on the aspects of cloud robotics: big data, cloud computing, collective robot learning and crowd-sourcing. 

Teleoperation mechanisms vary from game interfaces~\cite{marin2005multimodal} to free-space positioning interfaces~\cite{kofman2005teleop}. A comparison of various control interfaces shows that general purpose hardware is deficient in while special purpose hardware while more accurate is not widely available~\cite{kent2017comparison, marin2005multimodal}. Recent focus on virtual reality based free-space controllers have been proposed both for data collection~~\cite{whitney2017comparing,lipton2018baxter} and policy learning~\cite{yan2017learning,zhang2017deep}. 
While these methods have shown the utility of data, yet they don't provide a seamlessly scalable data collection mechanism. Often the data is either collected locally or requires a powerful local client computer, to render the high definition sensor stream to a VR headset~\cite{whitney2017comparing, zhang2017deep}
The use of VR hardware and requirement of client-side compute resources has limited the deployment of these interfaces on crowd-sourcing platforms such as MTurk and Datatang. 

\sysAbbr proposes the use of iPhone based controller which provides the fluid 6-DoF free space control similar to a VR Controller, while being ubiquitous. In addition, we also develop a cloud run simulation framework to ensure homogeneous quality of service regardless of client's compute resources. \sysAbbr relaxes the requirement to have a heavy-duty local computer at the client node. 
The two components combined result in a platform that is intuitive to use, and has a low barrier to entry -- the core requirements of a crowdsourced task.


% A number of studies have shown the use of these systems for long-distance control of physical robots~\cite{manzi2016use} and in human-robot interaction~\cite{magyar2017cowooz}.

% Teleoperation of a Robot Manipulator Using a Vision-Based Human–Robot Interface \cite{kofman2005teleop}

% A Multimodal Interface to Control a Robot Arm via the Web: A Case Study on Remote Programming~\cite{marin2005multimodal}
% studies not only the teleoperation interfaces but also analyzes the network performance of the architecture. 


% Comparing Robot-centric and Human-centric demos
% https://arxiv.org/abs/1610.00850

% -Preferable to collect demonstrations and then have robot learn instead of interactive Dagger-style method.
% And collecting such amounts of data has been a challenge in robotics. 


% The Robotarium: A remotely accessible swarm robotics research testbed.
% Accessible through public web interface, can test variety of multi-robot algorithms.
% \cite{pickem2017robotarium}https://arxiv.org/abs/1609.04730


% Wizard of Oz Studies in HRI: A Systematic Review and New Reporting Guidelines
% https://pdfs.semanticscholar.org/8a97/4faff697d9843a8c75f6eb6a79ca3393098d.pdf
% -Overview of Wizard of Oz in HRI

% Bilateral teleoperation: An historical survey~\cite{hokayem2006bilateral}
% https://www.sciencedirect.com/science/article/pii/S0005109806002871

% Use Case Evaluation of a Cloud Robotics Teleoperation System ~\cite{manzi2016use}
% https://ieeexplore.ieee.org/document/7776604/


% CoWoOZ — A cloud-based teleoperation platform for social robotics
% \cite{magyar2017cowooz}


% VizWiz: Nearly Real-time Answers to Visual Questions
% http://up.csail.mit.edu/other-pubs/vizwiz.pdf

% -Phone interfaces for real-time answers.


% point-and-click interfaces \cite{leeper2012constraint}


% \textbf{Teleoperation / Crowdsourcing / Previous CCR-like works}
% On the contrary Teleoperation in robotics has been around since the early 60s. \tocite{}
% The advent of internet enabled long-distance communication, enabled some exciting explorations such as the Tele-garden installation. 

% Kinesthetic teaching is not intuitive and can result in unwanted
% visual artifacts [9], [11]. Using motion capture devices for
% teleoperation, such as [37], is more intuitive and can solve
% this issue.

%  In a non-learning setting, VR teleoperation has
% been recently explored for controlling humanoid robots ~\cite{fritsche2015first}, \cite{lipton2018baxter}, for simulated dexterous manipulation [43], and for
% communicating motion intent [44]. Existing use cases of VR
% for learning policies have so far been limited to collecting
% waypoints of low-dimensional robot states ~\cite{yan2017learning}, ~\cite{kumar2016learning}. 

% Using dVRK Teleoperation to Facilitate Deep Learning of Automation Tasks for an Industrial Robot
% \cite{liang2017using}

% Deep Imitation Learning for Complex Manipulation Tasks from Virtual Reality Teleoperation
% \cite{zhang2017deep}

% Communicating Robot Arm Motion Intent Through Mixed Reality Head-mounted Displays
% \cite{rosen2017communicating}

% -Tellex paper on mixed reality interfaces

% Comparing Robot Grasping Teleoperation across Desktop and Virtual Reality
% with ROS Reality
% \cite{whitney2017comparing}
% -Tellex paper on their VR system

% The Robot Management System:
% A Framework for Conducting Human-Robot
% Interaction Studies Through Crowdsourcing
% \cite{toris2014robot}

% -Sonia Chernova HRI framework

% A Comparison of Remote Robot Teleoperation
% Interfaces for General Object Manipulation
% \cite{kent2017comparison}

% -Sonia Chernova comparison of teleop interfaces


% \noindent \textbf{Cloud Robotics.}
% % The idea of cloud enabled robotics has been around for a few decades. 
% % Cloud robotics as a term was coined by James Kuffner in 2010, with the idea of large scale computing to offload CPU-heavy tasks to remote servers. 
% In 2010, James Kuffner coined the term “Cloud Robotics” and the idea of large scale computing to offload CPU-heavy tasks to remote servers~\cite{kuffner2010cloud}.  
% Kehoe et al.\cite{kehoe2014tase} provides an excellent treatise that touches on the aspects of cloud robotics: big data, cloud computing, collective robot learning and crowd-sourcing. 
% Similar overviews of cloud enabled robot systems for special applications such as SLAM have also been studied~\cite{doriya2017review}.  
% Grasping as a robotics primitive task has been particularly amenable to cloud-based automation. Cloud-based systems have been used for grasping with google object recognition engine~\cite{kehoe2013cloud}, and grasp analysis and training in simulation with google cloud~\cite{kehoe2015cloud,mahler2016dex}.


% A number of efforts have attempted broader efforts to realize the benefits of cloud. RoboEarth was proposed as``a World Wide Web for robots: a giant network and database repository where robots can share information and learn from each other about their behavior and environment"~\cite{waibel2011roboearth}. It evolved into a commercial cloud platform: Rapyuta~\cite{mohanarajah2015rapyuta}. Similar efforts were pursued with DaVinci~\cite{arumugam2010davinci} and RoboBrain~\cite{arumugam2010davinci} as knowledge engines for robot clients. 
% \todo{how is \sys different}




% State of-the-art
% teleoperation systems require the operator to both manage their view of
% the scene and, separately, command the robot’s actuators. This is typically performed
% with keyboard and mouse interfaces, as was the case for the DARPA
% Robotics Challenge [13].



%  While there have been a few systems
% that enable robot teleoperation using VR [4, 3, 2], these systems did not provide
% the fluid camera control and handtracking movement, and their performance has not
% been evaluated empirically.



% the systems are often built for small set of data. 

% The core task of a VR visualization system is creating a realistic and natural visualization
% of the environment—fusing sensor data, joint positions, and available object
% and robot models—that responds to the operator’s movements in real time, without
% disorienting lag. 



==> 5-learning-expt.tex <==
\vspace{-12pt}
\section{Experiments}

\vspace{-5pt}
\subsection{Large-scale Data Collection}
\vspace{-5pt}
As an initial pilot for our system, we collected a dataset of over 1000 demonstrations on each of the bin sorting and peg-in-hole tasks with 20 hours of total system usage by using contractors that were located remotely. Indeed, this validates the idea that \Sys{} is truly a dynamic data collection system that can be used to quickly crowdsource data on-demand. The appendix contains some additional information and statistics on the dataset. 

%We note that the contracted demonstrations were not as consistently fast as our in-house experiments. This is likely due to the fact that we have tested this system through development so we are much more experienced in manipulation than fresh workers. However, we were able to generate a much larger quantity of data with these workers, and their demonstrations still yielded good results. 

% \begin{figure}[!t]
% \centering
%   \includegraphics[width=0.8\linewidth]{figures/insert.png}
%   \caption{Time taken to grasp and place the four different types of objects in the bin picking task across all users in the large-scale dataset.}
%   \label{fig:large_scale_objects}
%   \vspace{-20pt}
% \end{figure}

\vspace{-5pt}
\subsection{Learning Results}
\vspace{-5pt}

\todo{Update this with the latest results, once they are available...}

We evaluate several methods of learning control policies for the manipulation tasks, including reinforcement learning methods that rely on a reward function, imitation learning methods that learn from human demonstrations, and hybrid models that combine reinforcement learning and imitation learning. For reinforcement learning, we use a distributed version of proximal policy optimization (DPPO)~\cite{heess2017emergence} to learn from the reward functions defined on the tasks. For imitation learning, we offer comparisons of two different types of methods: a non-parametric baseline (NP) that performs nearest neighbor search based on the physical states and executes the corresponding actions in the nearest neighbor of the demonstration dataset and a behavior cloning (BC) baseline that trains a policy with supervision of the state-action pairs in the demonstration dataset using $\ell_2$-loss. For hybrid models, we evaluate two strategies as well: the Generative Adversarial Imitation Learning (GAIL)~\cite{ho2016generative} with reward augmentation, which combines the GAIL reward and environment reward, and the demonstration curriculum strategy~\cite{kakade2002approximately,popov2017data,zhu2018reinforcement} (DPPO\,+\,Demo) which uses demonstration states to randomly initialize training episodes along the demonstration trajectories and performs forward RL with distributed PPO.

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.4]{figures/cans-from-demos-v2.png}
%     \caption{PPO performance on bins easy bootstrapped with demonstrations }
%     \label{fig:cans-from demos}
% \end{figure}

% \begin{figure}
% \begin{tabular}{ |c|c|c||c|c| } 
% \hline
% Algorithm & Bins Can & Bins Hard &Pegs Round & Pegs Hard \\
% \hline
%  Baseline& s & 12.7022 & -  & 23.5643 \\ 
%  BC& 1.238 & - & 4.2173 & - \\
%  RL& 14.58  & 570.35 & -  & 148.34 \\  
%  RL + demos& 163.37$^*$ & 95.86 & 208.27$^*$  & 85.21 \\ 
% \hline
% \end{tabular}
% \caption{ Comparison of learning methods. Tasks marked with a $^*$ are solved}
% \end{figure}

\begin{figure*}[!t]
\centering
\begin{minipage}[c]{.55\linewidth}
    \centering
    \label{fig:numebrs}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{ll||llll}
    \hline
    \rowcolor[HTML]{CBCEFB} 
    Method & Algorithm                        & Bins Can & Bins Hard & Pegs Round & Pegs Hard \\ \hline
    \cellcolor[HTML]{FFCC67}RL & \cellcolor[HTML]{CBCEFB}DPPO       &  2.92    &  \textbf{7.13}   &  -    &   1.85    \\ \hline
    \cellcolor[HTML]{FFCC67}IL & \cellcolor[HTML]{CBCEFB}NP &    3.64    & 0.299      &     3.36       &   0.17        \\
    \rowcolor[HTML]{EFEFEF} 
    \cellcolor[HTML]{FFCC67}IL & \cellcolor[HTML]{CBCEFB}BC       & 0.24 & 0.0188 &   0.84    &  0.055 \\ \hline
    \rowcolor[HTML]{EFEFEF}
    \cellcolor[HTML]{FFCC67}RL+IL & \cellcolor[HTML]{CBCEFB}GAIL %$^{\dagger}$
    & 0.968 & 0.83 & 8.30 & \textbf{3.91} \\
    \rowcolor[HTML]{EFEFEF} 
    \cellcolor[HTML]{FFCC67}RL+IL & \cellcolor[HTML]{CBCEFB}DPPO\,+\,Demo &  \textbf{32.68*}    &   1.20    &   \textbf{41.66*}   &  1.065  \\ \hline 
    \end{tabular}
}

% \begin{figure*}[!t]
% \centering
% \begin{minipage}[c]{.55\linewidth}
%     \centering
%     \label{fig:numebrs}
%     \resizebox{0.95\linewidth}{!}{%
%     \begin{tabular}{ll||llll}
%     \hline
%     \rowcolor[HTML]{CBCEFB} 
%     Method & Algorithm                        & Bins Can & Bins Hard & Pegs Round & Pegs Hard \\ \hline
%     \cellcolor[HTML]{FFCC67}RL & \cellcolor[HTML]{CBCEFB}DPPO       &  14.6    &  570.4   &  -    &   148.3    \\
%     \cellcolor[HTML]{FFCC67}IL & \cellcolor[HTML]{CBCEFB}NP &    18.2    & 23.9      &     16.8       &   13.6        \\
%     \rowcolor[HTML]{EFEFEF} 
%     \cellcolor[HTML]{FFCC67}IL & \cellcolor[HTML]{CBCEFB}BC       & 1.2 & 1.5 &   4.2    &  4.4 \\
%     \rowcolor[HTML]{EFEFEF}
%     \cellcolor[HTML]{FFCC67}RL+IL & \cellcolor[HTML]{CBCEFB}GAIL %$^{\dagger}$
%     & - & 66.4 & - & 312.8 \\
%     \rowcolor[HTML]{EFEFEF} 
%     \cellcolor[HTML]{FFCC67}RL+IL & \cellcolor[HTML]{CBCEFB}DPPO\,+\,Demo &  163.4*    &   95.9    &   208.3*   &  85.2  \\ \hline 
%     \end{tabular}
% }

% \begin{figure*}[!t]
% \centering
% \begin{minipage}[c]{.55\linewidth}
%     \centering
%     \label{fig:numebrs}
%     \resizebox{0.95\linewidth}{!}{%
%     \begin{tabular}{l||llll}
%     \hline
%     \rowcolor[HTML]{CBCEFB} 
%     Algorithm                        & Bins Can & Bins Hard & Pegs Round & Pegs Hard \\ \hline
%     \cellcolor[HTML]{FFCC67}NP &    18.2    & 23.9      &     16.8       &   13.6        \\
%     \rowcolor[HTML]{EFEFEF} 
%     \cellcolor[HTML]{FFCC67}BC       & 1.2 & 1.5 &   4.2    &  4.4 \\
%     \rowcolor[HTML]{EFEFEF}
%     \cellcolor[HTML]{FFCC67}GAIL %$^{\dagger}$
%     & - & 66.4 & - & 312.8 \\
%     \cellcolor[HTML]{FFCC67}DPPO       &  14.6    &  570.4   &  -    &   148.3    \\
%     \rowcolor[HTML]{EFEFEF} 
%     \cellcolor[HTML]{FFCC67}DPPO\,+\,Demo &  163.4*    &   95.9    &   208.3*   &  85.2  \\ \hline 
%     \end{tabular}
% }
\end{minipage}%
\begin{minipage}[c]{.445\linewidth}
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.7\linewidth]{figures/cans-from-demos.png}
    % \caption{}
    % \caption{We evaluated our system on three simulated manipulation tasks which contain a 7-DOF Sawyer robot arm and various objects. The tasks were implemented using the MuJoCo physics engine. In the lifting task (a) the objective is to control the robot arm to grab the cube and lift it up. In the bin sorting task (b) the objective is to place each object into its corresponding bin. In the peg-in-hole task (c), the objective is to place a round nut and square nut onto their corresponding pegs. These screenshots were taken along successful demonstrations of each of the tasks.}
    % \label{fig:cans-from demos}
\end{minipage}%
\caption{\textbf{Learning}: Comparison of various learning methods in the manipulation tasks. In the table on the left, the runs marked as * imply that the task is solved. We observe that the methods achieve the highest episode rewards when combining reinforcement learning aided by the human demonstrations collected by \Sys{}. On the right we see that the learning algorithms benefit from an increasing number of demonstrations. }
\label{fig:cans-from-demos}
\vspace{-20pt}
\end{figure*}

We report the results in the table and training curves presented in Fig.~\ref{fig:cans-from-demos}. Forward reinforcement learning (DPPO) with random exploration is insufficient to solve even the easy version of the bins and pegs task limited to always spawning a single type of object. The simple imitation learning methods, NP and BC, can sometimes learn to reach the objects; however, they do not have enough capacity to consume demonstrations with great variations. The best performance is given by the methods (GAIL and DPPO\,+\,Demo) that effectively leverage demonstration data while still interacting with the environment via trial and error. We also note that diverse demonstrations help the learning agent diversify= state visitation and guide it to explore high-reward states. DPPO\,+\,Demo, aided by the demonstrations we collected, is the only method that is able to solve the easy tasks.


% We presented some results on a distributed reinforcement learning framework for utilizing demonstrations collected from our system and showed that the data enables policy learning on a couple of easier version of our tasks. 

From our initial findings, the dataset we collected motivates new challenges in imitation and reinforcement learning on how to use large amounts of demonstration data that is not necessarily optimal. The only guarantee we have on the demonstration data is that the user completed the task, but they could have taken sub-optimal trajectories. Our final model is a very simple way to utilize the demonstrations by controlling the start state distribution that the agent sees during training. We envision that more sophisticated algorithms can better leverage the demonstrations we collected. Our results also show that there is value in our system's ability to collect large quantities of demonstration data, both in terms of the number of environment interactions required and in terms of final performance. A large and diverse dataset of demonstrations can encourage the agent to explore and learn more effectively.



% To combat the exploration problem we bias the start state distribution of the environment towards states encountered in demonstrations similar to \cite{}. Doing this allows our agent to experience high reward states that it would not have if doing just random exploration. With a probability $\epsilon$ we sample a start state uniformly at random from the collected demonstrations and with the remaining probability init to the true start state of the environment. As is evident from \ref{fig:cans-from demos} even such a simple method to bootstrap exploration using demonstrations is able to solve the easy version of the bins task whereas just reinforcement learning was unable to and also note that using a 


%\subsubsection{Results on data we collected ourselves}

%\todo{Compare having 1, 10, 100, 1000 demos}
%
%Algos
%
%%BC
%GAIL (with BC init?)
%GAIL (with env rewards)
%Surreal PPO
%Surreal PPO with demos
%
%Tasks (should we have shaping vs. no shaping?)
%
%Bins (single)
%Bins (easy)
%Bins (hard) 
%
%Pegs (single)
%Pegs (easy)
%Pegs (hard)
%
%
%Learning results on U.S. vs. China (everything but PPO)
%
%We should also have a plot comparing algos with number of demos (1, 10, 100, 1000)
